Polar planets around highly eccentric binaries are the most stable

We study the orbital stability of a non-zero mass, close-in circular orbit planet around an eccentric orbit binary for various initial values of the binary eccentricity, binary mass fraction, planet mass, planet semi--major axis, and planet inclination by means of numerical simulations that cover $5 \times 10^4$ binary orbits. For small binary eccentricity, the stable orbits that extend closest to the binary (most stable orbits) are nearly retrograde and circulating. For high binary eccentricity, the most stable orbits are highly inclined and librate near the so-called generalised polar orbit which is a stationary orbit that is fixed in the frame of the binary orbit. For more extreme mass ratio binaries, there is a greater variation in the size of the stability region (defined by initial orbital radius and inclination) with planet mass and initial inclination, especially for low binary eccentricity. For low binary eccentricity, inclined planet orbits may be unstable even at large orbital radii (separation $> 5 \,a_{\rm b}$). The escape time for an unstable planet is generally shorter around an equal mass binary compared with an unequal mass binary. Our results have implications for circumbinary planet formation and evolution and will be helpful for understanding future circumbinary planet observations.

==> response-new.tex <==
Dear Scientific Editor and Assistant Editor,
We thank the referee for pointing out the issue with Eq. 3.
Equation 3 in Chen et al (2019) was missing +90. In both that paper and this one,the vectors in that equation should be unit vectors. These typos that did not affect the results of our calculations. We will submit an erratum for the Chen et al. (2019) paper. We also enlarged font sizes of the label, tick, and title in each figure and hope that you are satisfied with the revised manuscript.

Sincerely,
Cheng Chen, Stephen H. Lubow & Rebecca G. Martin.

==> response.tex <==
Dear Scientific Editor and Assistant Editor,
We thank the referee for the useful report that has improved the manuscript.
We have thoroughly reviewed the referee’s comments and made several
changes to the manuscript. Referee-prompted changes in the updated
document are highlighted in bold text. Additional edits, clarifying our
methodology and results, are included, but not highlighted. We hope that you
are satisfied with the revised manuscript.
Sincerely,
Cheng Chen, Stephen H. Lubow & Rebecca G. Martin.

Comments and suggestions:

Q1. Sect. 1, 1st paragraph: Out of curiosity, based on recent surveys, is there a correlation between “the break between alignment and misalignment of CBDs with the central binary” (at $T_b$ ~ 30 days) and the stellar mass?

CC: According to Table 3 ~ 4 in Czekala (2019), the binary systems which they choose have a wide range of the stellar masses. Besides, Table 5. in the same paper, there are 26 CBDs with unknown orientations. Thus, it hard to say any correlation between alignment and misalignment of CBDs with the central binary” (at $T_b$ ~ 30 days) unless we have more confirmed data.

Q2. Sect. 1, 3rd paragraph: I would strongly suggest to add a reference to Martin & Triaud (2014) regarding the transit probability.

CC: We added this reference in the end of 3rd paragraph in Sect. 1.

Q3. Sect. 1: There are a couple of recents works (Cuello & Giuppone 2019, Giuppone & Cuello 2019) where they explore the orbital dynamics of massive P-type planets around eccentric binaries that should be mentioned here.

CC: We mentioned and added these references in the last paragraph of Section 1.

Q4. Figs. 1, 2, 3, 4, 5 and 6: I would suggest to add labels (e.g. “A1, $e_b$=0.2, $f_b$=0.5, $m_p$=0.001) as in Chen et al. (2019). That would help to reader to go through the maps and better extract the information displayed.

CC: We have followed the reviewer’s suggestion and added labels for each plot.

Q5. Sect. 2.2: Typo “at the from red-purple boundary”. Remove “from”.

CC: We fixed the typo in this sentence

Q6. As a general comment, would it be possible to compute the Mean Exponential Growth of Nearby Orbits (MEGNO) indicator (Cincotta & Simó 2000) for the orbits considered? In this work, an orbit is defined as stable if it verifies the three criteria of Sect. 2.1. However, I suspect that some of these stable orbits might be chaotic and this could be easily identified at low CPU-cost.

CC: There is a built-in MEGNO function in REBOUND. To test how stable our simulations are, we considered the most extreme case with $f_{\rm b}$ = 0.1, $e_{\rm b}$ = 0.8 and $m_{\rm p}$ = 0.01 $m_{\rm b}$ (Model C6) with the high accuracy IAS15 integrator and the stability map shows most of stable orbits have MEGNO indicators = 2. The MEGNO stability map in the new Fig. 5 is similar
to our results in the lower right panel of Fig 2. In any case, it agrees with
our main result that the generalised polar orbits are the most stable 
for high binary eccentricity.


Q7. Sect. 2.2.2: Regarding the effect of the binary mass ratio on the stability of the planet, Cuello & Giuppone (2019) reported dynamical maps for polar orbits for massive planets with chaotic regions. They find that polar circumbinary planets around eccentric binaries are less stable for low binary mass ratios (see their Figure 8). This should be commented here.

CC: We added sentences to discuss this at the end of Sect. 2.2.2.   

Q8. Sect. 2.2 last paragraph: Add a reference to Giuppone & Cuello (2019) where it is shown that “the orbits are generally more unstable for the low mass fraction binary compared to the case of an equal mass binary” (see for instance their Figure 3).

CC: We missed “polar” in the sentence and a complete sentence is “the polar orbits are generally more unstable for the low mass fraction binary.”

Q9. Figs. 5 and 6: Since these plots are inspired by Figure 15 in Doolin & Blundell (2011) I would strongly suggest to add a colour code in order to identify different types of orbits: prograde, retrograde, and polar.

CC: We tried to make Figs. 5 and 6 in this way before. However, we found some unstable orbits meet the unstable conditions before it is possible to classify the type of orbit. For the test particle case in Doolin(2011), it is possible to classify because the critical inclination does not depend on semi-major axis of the particle. Therefore, to avoid this problem, we use the black and white colour bar instead of adding a colour code for these two figures.

Q10. Sect. 2.4: Is there a physical/analytical explanation for the long-lived unstable orbits observed for $f_b$ <= 0.1 (especially for large planetary masses in Figure 6).

CC: For more extreme mass ratio binaries, the binary torques due to resonances are weaker and therefore the unstable planet orbits evolve more slowly. We do not have an explanation for the behaviour with planet mass and inclination. We added a sentence  near the end of Section 2.4.

Q11. Sect. 3, 4th paragraph: I believe there is a missing reference regarding the resonant Lindblad torque of the binary on the circumbinary disc, for various values of e and i (Miranda & Lai 2015). This work was previously published to Lubow & Martin (2018) and Franchini et al (2019b) and should be cited here.

CC: We cited this reference in Sect. 3, 4th paragraph. However, note that
this effect of torque decreasing with e for i=90 is barely seen in Fig 12 of Miranda and Lai 2015 because their largest eccentricity was 0.7. Their problem was that they used a series expansion in e to evaluate the torque, while we computed the torque in Lubow and Martin 2018 without using an expansion in e.
We could then study the torque at larger e and show that it goes to zero as e goes to unity, as discussed further in Fanchini et al. 2019b.

Q12. I would strongly suggest to further discuss the astrophysical implications of this work, especially in the field of circumbinary planet dynamics and evolution. For instance, based on the results shown in Fig. 2, can the authors predict that very eccentric binaries should almost exclusively host polar circumbinary planets? Also, it seems that polar planets are less probable around unequal mass binaries, unless the binary eccentricity is >= 0.5. Assuming these statements are reasonable, I would like to see these discussed given the binary demographics available. In principle, the authors should be able to provide some predictions for future surveys.

CC: We added 2 paragraphs at the end of Sect. 3 that discuss predictions of close-in and far apart circumbinary planets. 

